Testing Assumptions Underlying a Unified Theory for the Origin of Grid Cells

Representing and reasoning about physical space is fundamental to animal survival, and the mammalian lineage expresses a wealth of specialized neural representations that encode space. Grid cells, whose discovery earned a Nobel prize, are a striking example: a grid cell is a neuron that fires if and only if the animal is spatially located at the vertices of a regular triangular lattice that tiles all explored two-dimensional environments. Significant theoretical work has gone into understanding why mammals have learned these particular representations, and recent work has proposed a ``unified theory for the computational and mechanistic origin of grid cells," claiming to answer why the mammalian lineage has learned grid cells. However, the Unified Theory makes a series of highly specific assumptions about the target readouts of grid cells - putatively place cells. In this work, we explicitly identify what these mathematical assumptions are, then test two of the critical assumptions using biological place cell data. At both the population and single-cell levels, we find evidence suggesting that neither of the assumptions are likely true in biological neural representations. These results call the Unified Theory into question, suggesting that biological grid cells likely have a different origin than those obtained in trained artificial neural networks.

==> tynybddgjtwfkdstmvyrwwjwqcbdnrcr/01_introduction.tex <==
\section{Introduction}

In the intricate realm of neural circuits that underpin navigation and spatial cognition, grid cells have emerged as an especially intriguing pattern of neuronal activity. Located in the mammalian medial entorhinal cortex, grid cells fire in a striking regular hexagonal grid pattern as an animal navigates through space \citep{hafting2005microstructure}. Their unique firing properties, believed to represent a metric for spatial navigation, have drawn extensive attention. Recent work proposed a new ``unified theory" for the origin of grid cells\footnote{In this context, ``theory" is intended in the sense of an accurate and predictive mathematical description of naturally occurring phenomena, akin to the theory of general relativity or quantum field theory.} \citep{sorscher_unied_2019, sorscher_unified_2020, sorscher_unified_2022, sorscher_when_2022} to answer \textit{why} the mammalian lineage has learned grid cells. However, the Unified Theory relies on a sequence of assumptions about grid cells performing supervised learning to predict specific targets, believed to be place cells (a type of neuron involved in spatial processing \citep{okeefe1971hippocampus,okeefe1976place,o1978hippocampal}).
To our knowledge, these assumptions have not been tested in  biological place cells. In this work, we seek to rectify this. We extract the assumptions made by the Unified Theory by revisiting its derivation in detail (App. \ref{app:theory}) then hone in on two pivotal suppositions specifically related to the readouts i.e. supervised targets of biological grid cells. We evaluate these assumptions against data from biological place cells and find that both assumptions are likely false. Such conclusions challenge the Unified Theory's explanation for the origin of grid cells in mammals.


==> tynybddgjtwfkdstmvyrwwjwqcbdnrcr/02_results.tex <==
\section{Results}

\paragraph{Identifying assumptions of the Unified Theory}

The Unified Theory seeks to answer why the mammalian lineage has learnt grid cells. Its answer is that grid cells are the optimal solution to predicting supervised targets that we generically call ``readouts". Earlier papers claimed that these readouts biologically correspond to place cells \citep{sorscher_unied_2019,sorscher_unified_2020}, although later papers \citep{sorscher_unified_2022, sorscher_when_2022} suggested that these readouts might correspond to other biological quantities (more later). We reproduce the Unified Theory in detail (App. \ref{app:theory}) to highlight its assumptions. In this work, we focus on two:
\begin{enumerate}
    \item The readouts, as a population, must be translationally invariant (Fig. \ref{fig:unified_theory_assumptions}, Left).
    \item The readouts, individually, must have carefully tuned center-surround tuning curves: either Difference-of-Softmaxes (DoS) or a particular Difference-of-Gaussians (DoG) tuning curve shape (Fig. \ref{fig:unified_theory_assumptions}, Right); these functions are defined in App. \ref{app:dos_and_dog}.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=0.30\textwidth,trim={7cm 1cm 4cm 0},clip]{figures/place_cell_centers_3d.pdf}%
    \includegraphics[width=0.30\textwidth,trim={7cm 1cm 4cm 0},clip]{figures/place_cell_3d_tuning_curve_pcindex=1.pdf}%
    \includegraphics[width=0.43\textwidth]{figures/place_cell_2d_tuning_curve_pcindex=1.pdf}
    \caption{\textbf{Two key assumptions of the Unified Theory.} Left: Readouts, as a population, must be translationally invariant. Center and Right: Readouts, individually, must have center-surround tuning curves.}
    \label{fig:unified_theory_assumptions}
\end{figure}


We focus on these two assumptions because they are mathematically critical for the Unified Theory's applicability to biological grid cells and numerically critical for deep recurrent neural networks to learn grid-like tuning \citep{banino_vector-based_2018, sorscher_unied_2019, sorscher_unified_2020, nayebi_explaining_2021, sorscher_unified_2022}, i.e., subsequent large-scale hyperparameter sweeps showed relaxing these assumptions causes disappearance of grid-like representations \citep{schaeffer_no_2022}.
To the best of our knowledge, these assumptions have not been quantitatively tested in biological data; we do so here.

\paragraph{Are place cells translationally invariant as a population?} In order to explain the origin of grid cells, the Unified Theory requires that the readouts possess a translation-invariant spatial autocorrelation structure (App. \ref{app:theory}): only if the readouts' spatial autocorrelation is (approximately) Toeplitz will its eigenvectors be (approximately) Fourier modes and thus induce periodic eigenvectors for emergence of grid-like tuning.
One reason to question this assumption is significant previous literature suggesting that place cells over-represent certain locations e.g., borders, landmarks, rewarded locations \citep{sato2020distinct,o1978hippocampal,wiener1989spatial,hetherington1997hippocampal,hollup2001accumulation,dupret2010reorganization,danielson2016sublayer,zaremba2017impaired, gauthier2018dedicated,bourboulou2019dynamic}.
Another reason is that place cells have a diversity of tuning curve widths, even at a single dorsoventral location, and even within individual cells as observed in recent experiments, e.g., \citep{eliav2021multiscale}; this work also theoretically and computationally shows that this dual heterogenous coding scheme is more optimal in terms of encoding position than a homogenous scheme, which underlies the assumptions of the Unified Theory and makes it unlikely to hold in biology.




We push the field forward by quantitatively measuring whether place cells are translationally invariant. We use calcium imaging of place cell populations from $320$ recording sessions across animals from \citep{lee2020statistical} and construct spatial autocorrelation matrices $\Sigma_i \defeq P_i P_i^T /n_p^{(i)}$, where $P_i \in \mathbb{R}^{n_x^{(i)} \times n_p^{(i)}}$ is the $i$th session's $n_p^{(i)}$ place cells' signals at $n_x^{(i)}$ spatial positions. To quantify how close a spatial autocorrelation matrix is to being Toeplitz, we define a matrix's projection onto the set of Toeplitz matrices $\mathcal{T}$:
%
\begin{equation}
\Pi_{\mathcal{T}}(\Sigma_i) \; \defeq \; \arg \min_{T \in \mathcal{T}} \big|\big|T - \Sigma_i \big|\big|_F^2. 
\label{eq:proj_to_toeplitz}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/pc_pop_structure.pdf}
    \caption{\textbf{Biological place cells populations are likely not translation invariant, as required mathematically by the Unified Theory.} Biological place cell populations from $320$ recorded sessions \citep{lee2020statistical} deviate significantly from a null distribution of translation-invariant artificial place cell population used to train deep networks, as measured by (A) the matrix distance (Kolmogorov-Smirnov 2-sample: $p=4.72\mathrm{e}{-5}$) and the (B) matrix absolute percent error (Kolmogorov-Smirnov 2-sample:  $p=1.44\mathrm{e}-87$). (C) Place cell spatial autocorrelation matrices $\Sigma_i$ do not visually display constant diagonals of Toeplitz matrices, as shown in 4 randomly chosen sessions. (D) Corresponding sessions' spatial autocorrelation matrices have non-periodic leading eigenvectors.} % XXX want a randomly shuffled version of the real and translationally invariant populations, to show that the non-uniformity seen in recording is more than you'd expect as simple standard deviation from a uniform random process. %XXX please confirm that you're re-setting all your default plotting to have larger numbers on the axes before proceeding for even another minute on any other work on this and other manuscripts!
    \label{fig:place_cell_pop_trans_invar}
\end{figure}

For details, see App. \ref{app:sec:toeplitz_projection}.
In each of the $320$ sessions, we subsample the largest continuous spatial region over which the population's summed activity is above some threshold $> 0$, construct $\Sigma_i$, then measure two different quantities to capture the extent to which the autocorrelation matrices deviates from being Toeplitz: (i) the matrix distance $\big|\big|\Pi_{\mathcal{T}}(\Sigma_i) - \Sigma_i \big|\big|_F$ and (ii) the matrix absolute percent error $\big|\big|\Pi_{\mathcal{T}}(\Sigma_i) - \Sigma_i \big|\big|_F/\big|\big|\Sigma_i \big|\big|_F$.
Because our goal is to test whether biological place cells match the artificial ``place cells" used to the train the networks, we constructed a null distribution based on the artificial ``place cells" used to in previous papers \citep{sorscher_unied_2019, sorscher_unified_2020, nayebi_explaining_2021, sorscher_unified_2022}.
Specifically, we created a translation-invariant artificial place cell population comprised of 15000 single-field, single-scale, ideal-width DoG readouts, then, for each session, we randomly subsampled artificial place cells' activity $\hat{P}_i$ matching the dimensions (i.e. number of spatial bins, number of neurons) of the biological place cell activity $P_i$, computed the artificial spatial autocorrelation $\hat{\Sigma}_i \defeq \hat{P}_i \hat{P}_i^T / n_p^{(i)}$, and measured the same two error metrics for $\hat{\Sigma}_i$.
After this has been done for all $320$ sessions, we apply a 2-sample Kolmogorov-Smirnov test \citep{massey1951kolmogorov} to both metrics under the null hypotheses that the biological and artificial empirical distributions were drawn from the same distribution.



For both metrics, and for all tested thresholds of spatial region coverage, biological responses have correlation structures that deviate significantly from the requisite Toeplitz structure (Fig. \ref{fig:place_cell_pop_trans_invar}AB). Specifically, we find the probability that biological place cell spatial autocorrelation matrices comes from the same distribution as the artificial translation-invariant autocorrelation matrices is, per the matrix distance, $4.72\mathrm{e}-5$  (Fig. \ref{fig:place_cell_pop_trans_invar}A) and, per the matrix absolute percent error, $1.44\mathrm{e}-87$ (Fig. \ref{fig:place_cell_pop_trans_invar}B). As further confirmation, the spatial autocorrelation matrices do not visually display the constant diagonals of Toeplitz matrices (Fig. \ref{fig:place_cell_pop_trans_invar}C), and the leading eigenvectors of the biological spatial autocorrelation matrices are not periodic (Fig. \ref{fig:place_cell_pop_trans_invar}D). These results suggest that biological place cell populations likely lack the translation invariance required by the Unified Theory.


\paragraph{Do place cells or their subthreshold responses have DoS or particular DoG shapes?}


In order to explain the origin of grid cells, the Unified Theory requires that the readouts of the grid cells must individually exhibit DoS or a particular DoG tuning curve shapes (App. \ref{app:theory}).
However, when testing this on biological data, there is some ambiguity: what are the readouts of biological grid cells?
Earlier papers \citep{banino_vector-based_2018, sorscher_unied_2019, sorscher_unified_2020, nayebi_explaining_2021, sorscher_unified_2022} referred to the readouts as place cells, e.g., Section 2 of \citep{sorscher_unied_2019} and Figure 1 of \citep{sorscher_unified_2022}.
However, biological place cells do not possess DoS/DoG-shaped tuning curves, as can been seen from the wealth of extracellular place cell electrophysiology results \citep{diba_forward_2007,okeefe1971hippocampus,okeefe1976place,wilson1993dynamics, foster2006reverse,duvelle2021hippocampal,mehta2000experience}.


\begin{figure}
\centering
\includegraphics[width= 0.75\textwidth]{figures/pc_dos.pdf}

\caption{{\bf Subthreshold voltages of place cells do not display DoG/DoS tuning.} (a-g) Measured membrane voltage from a selection of place cells in various conditions. Panels a-d reproduced from \cite{harvey2009}, e-f reproduced from \cite{bittner2017} and g reproduced from \cite{zhao2022} with permission. %(h) Position-position correlation matrices from a population of place cells on a 1d track from \citep{lee2020statistical} do not show translational invariance. Matrices aligned so that $(x-x')=0$ is along the vertical central line; translation invariance would correspond to mirror symmetry across the vertical. (i) Top 15 eigenvectors of the spatial autocorrelation matrix of a population of place cells in a 2d room from \citep{alme2014place} are not periodic (note that the top few eigenvectors are invariant to subsampling cells, dropping XXX\% of the cells -- suggesting that this inhomogeneity in the top eigenvectors is not a result of non-uniform place cell sampling).}
}
\label{fig:subthreshold_place_cell}
\end{figure} 

A second possibility later suggested by the Unified Theory
is that the readouts are \textit{subthreshold inputs to place cells from grid cells} \citep{sorscher_unified_2022,sorscher_when_2022}, though it is difficult to imagine why or how the target for the entorhinal grid cells would be a particular shape of {\em subthreshold} activation function of downstream neurons.
To test this possibility, we hunted down and collated intracellular voltage recordings of CA1 place cells \citep{harvey2009,bittner2017,zhao2022} (Fig. \ref{fig:subthreshold_place_cell}).
These recordings do not reveal DoS/DoG-shaped subthreshold responses near their place fields.
These results suggest that place cell inputs likely lack the center-surround shape required by the Unified Theory and used numerically \citep{sorscher_unied_2019,sorscher_unified_2020, nayebi_explaining_2021, sorscher_unified_2022}.
A third possibility suggested by the Unified Theory is that readouts are summed grid cell contribution to inputs to place cells; we do not know of any dataset or experimental technique through which this claim could be tested.
 


==> tynybddgjtwfkdstmvyrwwjwqcbdnrcr/03_discussion.tex <==
\section{Discussion}

In this work, we test two assumptions made by the Unified Theory for the origin of grid cells and found both are likely not true at both the population and single cell levels. Our results call the Unified Theory into question, suggesting that biological grid cells likely have a different origin than the grid-like representations found in trained artificial neural networks \citep{banino_vector-based_2018, cueva_emergence_2018, sorscher_unied_2019}.
For a more promising alternative, see \cite{schaeffer2023self}.

